A Reproducible and Realistic Evaluation of Partial Domain Adaptation Methods

Unsupervised Domain Adaptation (UDA) aims at classifying unlabeled target images leveraging source labeled ones. In this work, we consider the Partial Domain Adaptation (PDA) variant, where we have extra source classes not present in the target domain. Most successful algorithms use model selection strategies that rely on target labels to find the best hyper-parameters and/or models along training. However, these strategies violate the main assumption in PDA: only unlabeled target domain samples are available. Moreover, there are also inconsistencies in the experimental settings - architecture, hyper-parameter tuning, number of runs - yielding unfair comparisons. The main goal of this work is to provide a realistic evaluation of PDA methods with the different model selection strategies under a consistent evaluation protocol. We evaluate 7 representative PDA algorithms on 2 different real-world datasets using 7 different model selection strategies. Our two main findings are: (i) without target labels for model selection, the accuracy of the methods decreases up to 30 percentage points; (ii) only one method and model selection pair performs well on both datasets. Experiments were performed with our PyTorch framework, BenchmarkPDA, which we open source.

==> tables/table_office_home_results_tasks.tex <==
\begin{table}[h]\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{c@{\hskip 3pt}|c@{\hskip 3pt}|c@{\hskip 3pt}|c@{\hskip 3pt}|c@{\hskip 3pt}|c@{\hskip 3pt}|c@{\hskip 3pt}|c@{\hskip 3pt}|c@{\hskip 3pt}|c@{\hskip 3pt}|c@{\hskip 3pt}|c@{\hskip 3pt}|c@{\hskip 3pt}|c@{\hskip 3pt}|c}
\textsc{Metric} & \textsc{Method} & AC & AP & AR & CA & CP & CR & PA & PC & PR & RA & RC & RP & Avg\\
\midrule\midrule
\multirow{7}{*}{\textsc{s-acc}} & \textsc{s. only} & 45.03 & 68.01 & 78.70 & 55.68 & 57.37 & 64.48 & 58.10 & 38.49 & 75.56 & 68.63 & 45.67 & 75.93 & 60.97\\
 & \textsc{pada} & 49.35 & 66.29 & 79.39 & 57.85 & 56.99 & 68.18 & 60.06 & 45.83 & 76.48 & 68.87 & 55.00 & 79.25 & 63.63\\
 & \textsc{safn} & 48.12 & 67.21 & 77.43 & 57.39 & 57.14 & 65.30 & 59.41 & 42.85 & 74.69 & 68.69 & 50.63 & 76.38 & 62.10\\
 & \textsc{ba3us} & 53.07 & 73.18 & 78.87 & 66.91 & 65.64 & 70.20 & 68.78 & 54.71 & 81.85 & 73.34 & 54.41 & 84.58 & 68.79\\
 & \textsc{ar} & 51.12 & 72.79 & 77.91 & 63.21 & 60.54 & 72.76 & 63.39 & 48.36 & 78.02 & 70.00 & 52.52 & 77.55 & 65.68\\
 & \textsc{jumbot} & 49.07 & 65.45 & 77.14 & 60.09 & 59.59 & 66.67 & 60.24 & 43.60 & 74.43 & 70.19 & 51.12 & 77.12 & 62.89\\
 & \textsc{mpot} & 53.07 & 72.61 & 78.50 & 61.92 & 64.16 & 70.22 & 64.13 & 50.87 & 77.40 & 70.40 & 53.99 & 77.61 & 66.24\\
\midrule\midrule
\multirow{7}{*}{\textsc{ent}} & \textsc{s. only} & 45.69 & 68.70 & 78.91 & 54.85 & 57.33 & 65.42 & 58.86 & 38.53 & 75.52 & 68.60 & 46.35 & 76.94 & 61.31\\
 & \textsc{pada} & 46.03 & 62.09 & 76.05 & 55.07 & 47.28 & 60.92 & 56.69 & 38.43 & 77.08 & 69.48 & 49.73 & 78.00 & 59.74\\
 & \textsc{safn} & 47.08 & 66.83 & 77.73 & 56.54 & 59.07 & 66.22 & 56.75 & 39.58 & 73.90 & 67.80 & 48.76 & 76.23 & 61.37\\
 & \textsc{ba3us} & 59.26 & 76.38 & 86.03 & 68.96 & 71.07 & 76.22 & 73.16 & 57.91 & 85.59 & 78.11 & 62.85 & 84.84 & 73.36\\
 & \textsc{ar} & 54.85 & 78.45 & 84.23 & 63.91 & 68.53 & 80.75 & 67.25 & 52.34 & 83.29 & 74.93 & 55.64 & 83.06 & 70.60\\
 & \textsc{jumbot} & 57.69 & 75.44 & 85.24 & 75.97 & 74.85 & 79.75 & 72.85 & 60.18 & 83.21 & 81.97 & 61.81 & 86.33 & 74.61\\
 & \textsc{mpot} & 52.94 & 68.94 & 75.98 & 60.58 & 65.99 & 71.51 & 58.28 & 49.87 & 73.77 & 64.98 & 57.53 & 73.17 & 64.46\\
\midrule\midrule
\multirow{7}{*}{\textsc{dev}} & \textsc{s. only} & 42.63 & 67.94 & 78.19 & 53.72 & 55.56 & 64.51 & 59.14 & 38.07 & 75.43 & 67.49 & 46.55 & 75.50 & 60.39\\
 & \textsc{pada} & 44.70 & 61.61 & 68.99 & 35.08 & 24.24 & 61.66 & 57.91 & 38.03 & 73.11 & 66.33 & 29.97 & 71.07 & 52.72\\
 & \textsc{safn} & 48.12 & 67.30 & 77.43 & 56.75 & 58.17 & 65.64 & 59.08 & 43.00 & 74.64 & 68.11 & 50.53 & 75.65 & 62.03\\
 & \textsc{ba3us} & 41.67 & 50.05 & 63.74 & 60.70 & 59.08 & 67.88 & 64.62 & 56.74 & 75.21 & 70.92 & 58.39 & 78.06 & 62.25\\
 & \textsc{ar} & 49.25 & 70.20 & 79.73 & 62.72 & 61.85 & 70.86 & 61.65 & 43.72 & 76.29 & 70.31 & 49.61 & 75.61 & 64.32\\
 & \textsc{jumbot} & 46.11 & 66.33 & 76.42 & 56.81 & 56.36 & 66.70 & 58.03 & 41.99 & 74.97 & 67.43 & 48.12 & 76.04 & 61.28\\
 & \textsc{mpot} & 46.07 & 65.43 & 76.46 & 56.44 & 57.95 & 66.35 & 57.64 & 43.60 & 74.86 & 67.68 & 48.12 & 75.89 & 61.37\\
\midrule\midrule
\multirow{7}{*}{\textsc{snd}} & \textsc{s. only} & 44.50 & 68.81 & 78.81 & 50.32 & 54.34 & 63.83 & 58.52 & 36.68 & 74.51 & 65.87 & 43.02 & 74.72 & 59.50\\
 & \textsc{pada} & 50.43 & 66.72 & 79.72 & 57.30 & 52.10 & 63.11 & 60.82 & 39.26 & 79.33 & 73.09 & 45.77 & 80.62 & 62.36\\
 & \textsc{safn} & 49.57 & 68.18 & 77.86 & 57.91 & 58.17 & 66.13 & 59.14 & 43.90 & 75.81 & 68.17 & 49.59 & 76.64 & 62.59\\
 & \textsc{ba3us} & 62.21 & 83.29 & 88.50 & 68.50 & 71.45 & 76.96 & 76.19 & 59.94 & 86.31 & 79.46 & 65.35 & 86.35 & 75.37\\
 & \textsc{ar} & 54.37 & 79.01 & 84.54 & 64.52 & 68.05 & 79.16 & 65.60 & 51.28 & 83.05 & 75.02 & 55.02 & 83.40 & 70.25\\
 & \textsc{jumbot} & 56.60 & 68.48 & 84.70 & 71.81 & 71.84 & 80.91 & 70.28 & 50.69 & 83.89 & 81.21 & 58.85 & 88.18 & 72.29\\
 & \textsc{mpot} & 32.96 & 49.73 & 57.39 & 44.11 & 38.66 & 50.06 & 43.74 & 28.66 & 58.40 & 56.90 & 39.34 & 63.14 & 46.92\\
\midrule\midrule
\multirow{7}{*}{\textsc{1-shot}} & \textsc{s. only} & 44.88 & 66.52 & 77.05 & 54.12 & 53.59 & 64.49 & 57.55 & 38.95 & 72.91 & 66.45 & 42.77 & 72.79 & 59.34\\
 & \textsc{pada} & 51.20 & 63.51 & 79.46 & 55.86 & 57.20 & 65.49 & 59.87 & 44.34 & 74.18 & 68.35 & 48.88 & 78.95 & 62.27\\
 & \textsc{safn} & 31.40 & 49.73 & 62.82 & 48.88 & 45.27 & 57.26 & 42.33 & 29.77 & 63.52 & 56.11 & 37.55 & 67.00 & 49.30\\
 & \textsc{ba3us} & 44.60 & 51.39 & 65.47 & 65.63 & 59.78 & 68.49 & 68.38 & 57.83 & 82.05 & 80.78 & 63.10 & 79.20 & 65.56\\
 & \textsc{ar} & 56.00 & 78.58 & 82.77 & 68.99 & 68.35 & 77.25 & 69.67 & 51.98 & 78.72 & 76.19 & 55.48 & 82.73 & 70.56\\
 & \textsc{jumbot} & 61.59 & 76.86 & 86.45 & 74.20 & 73.43 & 79.85 & 74.96 & 62.87 & 81.83 & 78.48 & 61.59 & 87.34 & 74.95\\
 & \textsc{mpot} & 53.97 & 68.78 & 78.04 & 69.24 & 65.88 & 71.42 & 70.31 & 53.03 & 76.88 & 76.52 & 57.39 & 77.95 & 68.28\\
\midrule\midrule
\multirow{7}{*}{\textsc{100-rnd}} & \textsc{s. only} & 43.60 & 69.45 & 78.70 & 55.19 & 57.11 & 65.64 & 59.14 & 39.22 & 75.87 & 68.53 & 45.63 & 77.20 & 61.27\\
 & \textsc{pada} & 50.41 & 67.21 & 79.97 & 56.69 & 53.86 & 63.94 & 60.27 & 40.56 & 78.91 & 72.70 & 53.39 & 80.73 & 63.22\\
 & \textsc{safn} & 47.58 & 67.53 & 77.91 & 56.47 & 58.19 & 65.88 & 59.69 & 43.14 & 75.00 & 69.64 & 50.85 & 76.41 & 62.36\\
 & \textsc{ba3us} & 62.53 & 82.09 & 88.28 & 69.15 & 71.65 & 77.21 & 75.15 & 58.17 & 85.92 & 79.86 & 66.57 & 85.66 & 75.19\\
 & \textsc{ar} & 54.89 & 78.54 & 84.34 & 64.95 & 69.00 & 79.57 & 66.73 & 50.85 & 82.39 & 74.66 & 55.42 & 82.80 & 70.34\\
 & \textsc{jumbot} & 61.07 & 77.87 & 86.01 & 74.56 & 76.40 & 81.54 & 72.60 & 59.92 & 84.63 & 81.85 & 64.84 & 87.64 & 75.74\\
 & \textsc{mpot} & 61.59 & 75.56 & 82.59 & 72.48 & 69.77 & 75.41 & 72.64 & 57.67 & 82.02 & 79.80 & 64.64 & 82.60 & 73.06\\
\midrule\midrule
\multirow{7}{*}{\textsc{oracle}} & \textsc{s. only} & 45.77 & 69.49 & 79.24 & 56.20 & 58.36 & 65.84 & 59.50 & 40.22 & 76.39 & 69.08 & 47.48 & 77.20 & 62.06\\
 & \textsc{pada} & 50.53 & 67.45 & 80.14 & 57.30 & 54.47 & 64.55 & 61.07 & 40.94 & 79.55 & 73.09 & 54.63 & 80.93 & 63.72\\
 & \textsc{safn} & 49.57 & 68.55 & 78.26 & 57.91 & 59.29 & 66.81 & 59.87 & 45.29 & 75.98 & 69.08 & 51.68 & 77.29 & 63.30\\
 & \textsc{ba3us} & 63.26 & 82.75 & 89.16 & 69.91 & 71.93 & 77.58 & 75.73 & 59.94 & 86.89 & 80.93 & 66.77 & 86.93 & 75.98\\
 & \textsc{ar} & 57.33 & 79.61 & 86.31 & 69.45 & 71.88 & 79.94 & 70.28 & 53.57 & 83.78 & 77.26 & 59.68 & 83.72 & 72.73\\
 & \textsc{jumbot} & 61.87 & 78.19 & 88.11 & 77.69 & 76.75 & 84.15 & 76.83 & 63.72 & 84.80 & 81.79 & 64.70 & 87.17 & 77.15\\
 & \textsc{mpot} & 64.48 & 80.88 & 86.78 & 76.22 & 77.95 & 82.59 & 75.18 & 64.60 & 84.87 & 80.59 & 67.04 & 86.52 & 77.31\\
\end{tabular}}
\caption{Accuracy on each of the 12 tasks of Partial Office-Home.}
\label{table:office_home_results_tasks}
\end{table}

==> tables/table_visda_results_tasks.tex <==
\begin{table}[h]\centering
\begin{tabular}{c@{\hskip 3pt}|c@{\hskip 3pt}|c@{\hskip 3pt}|c@{\hskip 3pt}|c}
\textsc{Metric} & \textsc{Method} & SR & RS & Avg\\
\midrule\midrule
\multirow{7}{*}{\textsc{s-acc}} & \textsc{s. only} & 45.91 & 63.51 & 54.71\\
 & \textsc{pada} & 44.56 & 50.39 & 47.48\\
 & \textsc{safn} & 52.04 & 64.37 & 58.20\\
 & \textsc{ba3us} & 44.21 & 65.99 & 55.10\\
 & \textsc{ar} & 68.39 & 64.97 & 66.68\\
 & \textsc{jumbot} & 55.23 & 66.04 & 60.63\\
 & \textsc{mpot} & 64.57 & 75.47 & 70.02\\
\midrule\midrule
\multirow{7}{*}{\textsc{ent}} & \textsc{s. only} & 49.10 & 61.20 & 55.15\\
 & \textsc{pada} & 40.83 & 23.80 & 32.32\\
 & \textsc{safn} & 48.05 & 58.72 & 53.38\\
 & \textsc{ba3us} & 71.17 & 59.99 & 65.58\\
 & \textsc{ar} & 75.28 & 53.26 & 64.27\\
 & \textsc{jumbot} & 56.25 & 68.59 & 62.42\\
 & \textsc{mpot} & 82.10 & 67.18 & 74.64\\
\midrule\midrule
\multirow{7}{*}{\textsc{dev}} & \textsc{s. only} & 47.00 & 63.61 & 55.30\\
 & \textsc{pada} & 41.04 & 45.82 & 43.43\\
 & \textsc{safn} & 52.42 & 64.82 & 58.62\\
 & \textsc{ba3us} & 48.78 & 68.01 & 58.40\\
 & \textsc{ar} & 68.54 & 65.86 & 67.20\\
 & \textsc{jumbot} & 54.35 & 65.36 & 59.86\\
 & \textsc{mpot} & 57.02 & 66.21 & 61.62\\
\midrule\midrule
\multirow{7}{*}{\textsc{snd}} & \textsc{s. only} & 51.17 & 60.18 & 55.68\\
 & \textsc{pada} & 56.14 & 57.53 & 56.83\\
 & \textsc{safn} & 43.90 & 60.59 & 52.24\\
 & \textsc{ba3us} & 46.12 & 56.01 & 51.07\\
 & \textsc{ar} & 57.61 & 53.78 & 55.69\\
 & \textsc{jumbot} & 75.23 & 80.16 & 77.69\\
 & \textsc{mpot} & 84.45 & 72.36 & 78.40\\
\midrule\midrule
\multirow{7}{*}{\textsc{1-shot}} & \textsc{s. only} & 49.43 & 62.35 & 55.89\\
 & \textsc{pada} & 52.94 & 53.36 & 53.15\\
 & \textsc{safn} & 49.97 & 63.82 & 56.89\\
 & \textsc{ba3us} & 66.79 & 62.75 & 64.77\\
 & \textsc{ar} & 71.08 & 69.59 & 70.34\\
 & \textsc{jumbot} & 81.27 & 75.42 & 78.34\\
 & \textsc{mpot} & 71.33 & 70.58 & 70.96\\
\midrule\midrule
\multirow{7}{*}{\textsc{100-rnd}} & \textsc{s. only} & 49.51 & 67.60 & 58.55\\
 & \textsc{pada} & 49.34 & 59.43 & 54.38\\
 & \textsc{safn} & 55.76 & 66.98 & 61.37\\
 & \textsc{ba3us} & 71.45 & 63.44 & 67.44\\
 & \textsc{ar} & 77.19 & 69.72 & 73.45\\
 & \textsc{jumbot} & 89.94 & 77.03 & 83.49\\
 & \textsc{mpot} & 87.25 & 84.96 & 86.11\\
\midrule\midrule
\multirow{7}{*}{\textsc{oracle}} & \textsc{s. only} & 51.41 & 67.60 & 59.50\\
 & \textsc{pada} & 49.34 & 59.81 & 54.57\\
 & \textsc{safn} & 56.88 & 68.40 & 62.64\\
 & \textsc{ba3us} & 71.77 & 63.56 & 67.67\\
 & \textsc{ar} & 77.73 & 70.23 & 73.98\\
 & \textsc{jumbot} & 90.55 & 77.46 & 84.01\\
 & \textsc{mpot} & 87.96 & 85.94 & 86.95\\
\end{tabular}
\caption{Accuracy on each of the 2 tasks of Partial VisDA.}
\label{table:visda_results_tasks}
\end{table}
